Deductive Additivity for Planning of Natural Language Proofs

Current natural language systems designed for multi-step claim validation typically operate in two phases: retrieve a set of relevant premise statements using heuristics (planning), then generate novel conclusions from those statements using a large language model (deduction). The planning step often requires expensive Transformer operations and does not scale to arbitrary numbers of premise statements. In this paper, we investigate whether an efficient planning heuristic is possible via embedding spaces compatible with deductive reasoning. Specifically, we evaluate whether embedding spaces exhibit a property we call deductive additivity: the sum of premise statement embeddings should be close to embeddings of conclusions based on those premises. We explore multiple sources of off-the-shelf dense embeddings in addition to fine-tuned embeddings from GPT3 and sparse embeddings from BM25. We study embedding models both intrinsically, evaluating whether the property of deductive additivity holds, and extrinsically, using them to assist planning in natural language proof generation. Lastly, we create a dataset, Single-Step Reasoning Contrast (SSRC), to further probe performance on various reasoning types. Our findings suggest that while standard embedding methods frequently embed conclusions near the sums of their premises, they fall short of being effective heuristics and lack the ability to model certain categories of reasoning.

==> Figs/ssrc_examples.tex <==
\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  analogy\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  A strong defense is essential for success in both football and military.\\
\textbf{Gold Premises}:  A football team needs a strong defense to win games. A military needs a strong defense to win battles.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  a football team needs a strong defense to win games. a military needs a strong defense to win battles.\\
\quad\textbf{Rank 2}:  a football team needs a strong defense to win games. all militaries without a strong defense always win battles.\\
\quad\textbf{Rank 3}:  a military needs a strong defense to win battles. football teams with weak defenses always win games.\\
\quad\textbf{Rank 4}:  all militaries without a strong defense always win battles. football teams with weak defenses always win games.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_0}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  analogy\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  A strong defense is essential for success in both football and military.\\
\textbf{Gold Premises}:  A football team needs a strong defense to win games. A military needs a strong defense to win battles.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  a military needs a strong defense to win battles. a football team needs a strong defense to win games.\\
\quad\textbf{Rank 2}:  a football team needs a strong defense to win games. military commanders who prefer coffee over tea are more successful in battle.\\
\quad\textbf{Rank 3}:  a football team needs a strong defense to win games. military units that have a team song tend to have higher morale.\\
\quad\textbf{Rank 4}:  military generals who have mustaches win more battles. a football team needs a strong defense to win games.\\
\quad\textbf{Rank 5}:  a military needs a strong defense to win battles. football teams that wear black uniforms win more games.\\
\quad\textbf{Rank 6}:  a military needs a strong defense to win battles. football teams that have a team mascot tend to win more games.\\
\quad\textbf{Rank 7}:  a military needs a strong defense to win battles. football teams with more instagram followers win more games.\\
\quad\textbf{Rank 8}:  football teams that wear black uniforms win more games. military commanders who prefer coffee over tea are more successful in battle.\\
\quad\textbf{Rank 9}:  football teams that wear black uniforms win more games. military units that have a team song tend to have higher morale.\\
\quad\textbf{Rank 10}:  football teams that have a team mascot tend to win more games. military commanders who prefer coffee over tea are more successful in battle.\\
\quad\textbf{Rank 11}:  football teams with more instagram followers win more games. military units that have a team song tend to have higher morale.\\
\quad\textbf{Rank 12}:  football teams with more instagram followers win more games. military commanders who prefer coffee over tea are more successful in battle.\\
\quad\textbf{Rank 13}:  football teams that wear black uniforms win more games. military generals who have mustaches win more battles.\\
\quad\textbf{Rank 14}:  football teams that have a team mascot tend to win more games. military units that have a team song tend to have higher morale.\\
\quad\textbf{Rank 15}:  military generals who have mustaches win more battles. football teams that have a team mascot tend to win more games.\\
\quad\textbf{Rank 16}:  football teams with more instagram followers win more games. military generals who have mustaches win more battles.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_1}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  analogy\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  A strong defense is essential for success in both football and military.\\
\textbf{Gold Premises}:  A football team needs a strong defense to win games. A military needs a strong defense to win battles.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  a military needs a strong defense to win battles. a football team needs a strong defense to win games.\\
\quad\textbf{Rank 2}:  a military needs a strong defense to win battles. some football teams need a strong defense to win games.\\
\quad\textbf{Rank 3}:  a football team needs a strong defense to win games. none of the militaries need a strong defense to win battles.\\
\quad\textbf{Rank 4}:  none of the militaries need a strong defense to win battles. some football teams need a strong defense to win games.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_2}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  analogy\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  A strong defense is essential for success in both football and military.\\
\textbf{Gold Premises}:  A football team needs a strong defense to win games. A military needs a strong defense to win battles.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  a football team needs a strong defense to win games. a military needs a strong defense to win battles.\\
\quad\textbf{Rank 2}:  not all militaries need a strong defense to win battles. a football team needs a strong defense to win games.\\
\quad\textbf{Rank 3}:  a military needs a strong defense to win battles. not all football teams need a strong defense to win games.\\
\quad\textbf{Rank 4}:  not all militaries need a strong defense to win battles. not all football teams need a strong defense to win games.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_3}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  categorical syllogism\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  Whiskers is an animal.\\
\textbf{Gold Premises}:  All cats are animals. Whiskers is a cat.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  all cats are animals. whiskers is a cat.\\
\quad\textbf{Rank 2}:  some cats are not mammals. whiskers is a cat.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_40}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  categorical syllogism\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  Whiskers is an animal.\\
\textbf{Gold Premises}:  All cats are animals. Whiskers is a cat.\\
\textbf{Rank}:  4\\
\quad\textbf{Rank 1}:  whiskers has a white spot on its paw. whiskers is a cat.\\
\quad\textbf{Rank 2}:  whiskers is a siamese cat. whiskers is a cat.\\
\quad\textbf{Rank 3}:  whiskers is a cat. whiskers has a collar with a bell on it.\\
\quad\textbf{Rank (G) 4}:  all cats are animals. whiskers is a cat.\\
\quad\textbf{Rank 5}:  whiskers is a siamese cat. whiskers is a rescue cat.\\
\quad\textbf{Rank 6}:  whiskers has a white spot on its paw. whiskers is a rescue cat.\\
\quad\textbf{Rank 7}:  whiskers is a siamese cat. whiskers likes to climb trees.\\
\quad\textbf{Rank 8}:  whiskers is a rescue cat. whiskers has a collar with a bell on it.\\
\quad\textbf{Rank 9}:  whiskers is a siamese cat. whiskers likes to sleep in the sun.\\
\quad\textbf{Rank 10}:  whiskers has a white spot on its paw. whiskers likes to climb trees.\\
\quad\textbf{Rank 11}:  all cats are animals. whiskers is a rescue cat.\\
\quad\textbf{Rank 12}:  whiskers likes to sleep in the sun. whiskers has a white spot on its paw.\\
\quad\textbf{Rank 13}:  whiskers likes to climb trees. whiskers has a collar with a bell on it.\\
\quad\textbf{Rank 14}:  whiskers likes to sleep in the sun. whiskers has a collar with a bell on it.\\
\quad\textbf{Rank 15}:  all cats are animals. whiskers likes to climb trees.\\
\quad\textbf{Rank 16}:  whiskers likes to sleep in the sun. all cats are animals.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_41}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  categorical syllogism\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  Whiskers is an animal.\\
\textbf{Gold Premises}:  All cats are animals. Whiskers is a cat.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  whiskers is a cat. all cats are animals.\\
\quad\textbf{Rank 2}:  whiskers is a cat. some cats are mammals.\\
\quad\textbf{Rank 3}:  some cats are mammals. whiskers is not a cat.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_42}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  categorical syllogism\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  Whiskers is an animal.\\
\textbf{Gold Premises}:  All cats are animals. Whiskers is a cat.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  all cats are animals. whiskers is a cat.\\
\quad\textbf{Rank 2}:  whiskers is a cat. some cats are not animals.\\
\quad\textbf{Rank 3}:  all cats are animals. whiskers is not a cat.\\
\quad\textbf{Rank 4}:  whiskers is not a cat. some cats are not animals.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_43}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  causal reasoning\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  John may become obese.\\
\textbf{Gold Premises}:  Eating too much junk food causes obesity. John eats a lot of junk food.\\
\textbf{Rank}:  3\\
\quad\textbf{Rank 1}:  eating too much healthy food causes obesity. john eats a lot of junk food.\\
\quad\textbf{Rank 2}:  eating too much junk food causes obesity. john eats a lot of healthy food.\\
\quad\textbf{Rank (G) 3}:  eating too much junk food causes obesity. john eats a lot of junk food.\\
\quad\textbf{Rank 4}:  eating too much healthy food causes obesity. john eats a lot of healthy food.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_78}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  causal reasoning\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  John may become obese.\\
\textbf{Gold Premises}:  Eating too much junk food causes obesity. John eats a lot of junk food.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  john eats a lot of junk food. eating too much junk food causes obesity.\\
\quad\textbf{Rank 2}:  john eats a lot of junk food. john wears glasses.\\
\quad\textbf{Rank 3}:  john is allergic to peanuts. john eats a lot of junk food.\\
\quad\textbf{Rank 4}:  john eats a lot of junk food. john has a cat named whiskers.\\
\quad\textbf{Rank 5}:  junk food is often advertised during sporting events. john wears glasses.\\
\quad\textbf{Rank 6}:  junk food is often sold in convenience stores. john wears glasses.\\
\quad\textbf{Rank 7}:  junk food is often sold in brightly colored packaging. john wears glasses.\\
\quad\textbf{Rank 8}:  junk food is often sold in brightly colored packaging. john is allergic to peanuts.\\
\quad\textbf{Rank 9}:  john is allergic to peanuts. junk food is often advertised during sporting events.\\
\quad\textbf{Rank 10}:  john has a cat named whiskers. junk food is often advertised during sporting events.\\
\quad\textbf{Rank 11}:  junk food is often sold in convenience stores. john is allergic to peanuts.\\
\quad\textbf{Rank 12}:  junk food is often sold in brightly colored packaging. john has a cat named whiskers.\\
\quad\textbf{Rank 13}:  junk food is often sold in convenience stores. john has a cat named whiskers.\\
\quad\textbf{Rank 14}:  eating too much junk food causes obesity. junk food is often advertised during sporting events.\\
\quad\textbf{Rank 15}:  junk food is often sold in brightly colored packaging. eating too much junk food causes obesity.\\
\quad\textbf{Rank 16}:  junk food is often sold in convenience stores. eating too much junk food causes obesity.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_79}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  causal reasoning\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  John may become obese.\\
\textbf{Gold Premises}:  Eating too much junk food causes obesity. John eats a lot of junk food.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  john eats a lot of junk food. eating too much junk food causes obesity.\\
\quad\textbf{Rank 2}:  john eats some junk food. eating too much junk food causes obesity.\\
\quad\textbf{Rank 3}:  john eats a lot of junk food. all junk food causes obesity.\\
\quad\textbf{Rank 4}:  john eats some junk food. all junk food causes obesity.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_80}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  causal reasoning\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  John may become obese.\\
\textbf{Gold Premises}:  Eating too much junk food causes obesity. John eats a lot of junk food.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  eating too much junk food causes obesity. john eats a lot of junk food.\\
\quad\textbf{Rank 2}:  eating too much junk food causes obesity. john doesn't eat a lot of junk food.\\
\quad\textbf{Rank 3}:  not all junk food causes obesity. john eats a lot of junk food.\\
\quad\textbf{Rank 4}:  not all junk food causes obesity. john doesn't eat a lot of junk food.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_81}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  classification\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  Apples, bananas, oranges, and grapes are all types of fruit.\\
\textbf{Gold Premises}:  Apples and bananas are types of fruit. Oranges and grapes are types of fruit.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  oranges and grapes are types of fruit. apples and bananas are types of fruit.\\
\quad\textbf{Rank 2}:  bananas and apples are not types of food. apples and bananas are types of fruit.\\
\quad\textbf{Rank 3}:  oranges and grapes are types of fruit. oranges and grapes are not fruits.\\
\quad\textbf{Rank 4}:  bananas and apples are not types of food. oranges and grapes are not fruits.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_118}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  classification\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  Apples, bananas, oranges, and grapes are all types of fruit.\\
\textbf{Gold Premises}:  Apples and bananas are types of fruit. Oranges and grapes are types of fruit.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  apples and bananas are types of fruit. oranges and grapes are types of fruit.\\
\quad\textbf{Rank 2}:  apples and bananas are types of fruit. grapes can be used to make wine.\\
\quad\textbf{Rank 3}:  apples are a common ingredient in apple pie. oranges and grapes are types of fruit.\\
\quad\textbf{Rank 4}:  oranges and grapes are types of fruit. apples are often used to make cider.\\
\quad\textbf{Rank 5}:  apples and bananas are types of fruit. bananas are often peeled before eaten.\\
\quad\textbf{Rank 6}:  oranges are a good source of vitamin c. oranges and grapes are types of fruit.\\
\quad\textbf{Rank 7}:  apples and bananas are types of fruit. bananas can be peeled from the top or bottom.\\
\quad\textbf{Rank 8}:  grapes can be used to make wine. oranges are a good source of vitamin c.\\
\quad\textbf{Rank 9}:  oranges are a good source of vitamin c. bananas are often peeled before eaten.\\
\quad\textbf{Rank 10}:  bananas can be peeled from the top or bottom. oranges are a good source of vitamin c.\\
\quad\textbf{Rank 11}:  bananas can be peeled from the top or bottom. apples are a common ingredient in apple pie.\\
\quad\textbf{Rank 12}:  grapes can be used to make wine. apples are a common ingredient in apple pie.\\
\quad\textbf{Rank 13}:  apples are a common ingredient in apple pie. bananas are often peeled before eaten.\\
\quad\textbf{Rank 14}:  bananas can be peeled from the top or bottom. apples are often used to make cider.\\
\quad\textbf{Rank 15}:  bananas are often peeled before eaten. apples are often used to make cider.\\
\quad\textbf{Rank 16}:  grapes can be used to make wine. apples are often used to make cider.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_119}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  classification\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  Apples, bananas, oranges, and grapes are all types of fruit.\\
\textbf{Gold Premises}:  Apples and bananas are types of fruit. Oranges and grapes are types of fruit.\\
\textbf{Rank}:  2\\
\quad\textbf{Rank 1}:  all apples and bananas are types of fruit. oranges and grapes are types of fruit.\\
\quad\textbf{Rank (G) 2}:  oranges and grapes are types of fruit. apples and bananas are types of fruit.\\
\quad\textbf{Rank 3}:  none of the oranges and grapes are types of fruit. apples and bananas are types of fruit.\\
\quad\textbf{Rank 4}:  all apples and bananas are types of fruit. none of the oranges and grapes are types of fruit.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_120}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  classification\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  Apples, bananas, oranges, and grapes are all types of fruit.\\
\textbf{Gold Premises}:  Apples and bananas are types of fruit. Oranges and grapes are types of fruit.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  oranges and grapes are types of fruit. apples and bananas are types of fruit.\\
\quad\textbf{Rank 2}:  not all oranges and grapes are types of fruit. apples and bananas are types of fruit.\\
\quad\textbf{Rank 3}:  oranges and grapes are types of fruit. not all apples and bananas are types of fruit.\\
\quad\textbf{Rank 4}:  not all oranges and grapes are types of fruit. not all apples and bananas are types of fruit.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_121}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  comparative reasoning\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  The blue car is faster than the yellow car.\\
\textbf{Gold Premises}:  The blue car is faster than the red car. The red car is faster than the yellow car.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the red car is faster than the yellow car. the blue car is faster than the red car.\\
\quad\textbf{Rank 2}:  the yellow car has a slower acceleration than the red car. the blue car is faster than the red car.\\
\quad\textbf{Rank 3}:  the blue car has a smaller engine than the red car. the red car is faster than the yellow car.\\
\quad\textbf{Rank 4}:  the blue car has a smaller engine than the red car. the yellow car has a slower acceleration than the red car.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_158}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  comparative reasoning\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  The blue car is faster than the yellow car.\\
\textbf{Gold Premises}:  The blue car is faster than the red car. The red car is faster than the yellow car.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the red car is faster than the yellow car. the blue car is faster than the red car.\\
\quad\textbf{Rank 2}:  the blue car has a sunroof. the red car is faster than the yellow car.\\
\quad\textbf{Rank 3}:  the yellow car has a sunroof. the blue car is faster than the red car.\\
\quad\textbf{Rank 4}:  the yellow car has leather seats. the blue car is faster than the red car.\\
\quad\textbf{Rank 5}:  the yellow car has a gps system. the blue car is faster than the red car.\\
\quad\textbf{Rank 6}:  the blue car has a full tank of gas. the red car is faster than the yellow car.\\
\quad\textbf{Rank 7}:  the blue car was once owned by a famous celebrity. the red car is faster than the yellow car.\\
\quad\textbf{Rank 8}:  the yellow car has a sunroof. the blue car has a full tank of gas.\\
\quad\textbf{Rank 9}:  the yellow car has a gps system. the blue car has a sunroof.\\
\quad\textbf{Rank 10}:  the blue car has a full tank of gas. the yellow car has leather seats.\\
\quad\textbf{Rank 11}:  the blue car has a full tank of gas. the yellow car has a gps system.\\
\quad\textbf{Rank 12}:  the yellow car has leather seats. the blue car has a sunroof.\\
\quad\textbf{Rank 13}:  the yellow car has a gps system. the blue car was once owned by a famous celebrity.\\
\quad\textbf{Rank 14}:  the yellow car has a sunroof. the blue car was once owned by a famous celebrity.\\
\quad\textbf{Rank 15}:  the yellow car has leather seats. the blue car was once owned by a famous celebrity.\\
\quad\textbf{Rank 16}:  the yellow car has a sunroof. the blue car has a sunroof.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_159}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  comparative reasoning\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  The blue car is faster than the yellow car.\\
\textbf{Gold Premises}:  The blue car is faster than the red car. The red car is faster than the yellow car.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the red car is faster than the yellow car. the blue car is faster than the red car.\\
\quad\textbf{Rank 2}:  the red car is faster than the yellow car. all blue cars are faster than red cars.\\
\quad\textbf{Rank 3}:  the blue car is faster than the red car. some yellow cars are slower than red cars.\\
\quad\textbf{Rank 4}:  some yellow cars are slower than red cars. all blue cars are faster than red cars.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_160}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  comparative reasoning\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  The blue car is faster than the yellow car.\\
\textbf{Gold Premises}:  The blue car is faster than the red car. The red car is faster than the yellow car.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the blue car is faster than the red car. the red car is faster than the yellow car.\\
\quad\textbf{Rank 2}:  the blue car is faster than the red car. the red car is not faster than the yellow car.\\
\quad\textbf{Rank 3}:  the red car is faster than the yellow car. the blue car is not faster than the red car.\\
\quad\textbf{Rank 4}:  the red car is not faster than the yellow car. the blue car is not faster than the red car.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_161}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  composition\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  The salad is healthy.\\
\textbf{Gold Premises}:  Every ingredient in a salad is healthy. A salad is made up of these ingredients.\\
\textbf{Rank}:  2\\
\quad\textbf{Rank 1}:  a salad is made up of these unhealthy ingredients. every ingredient in a salad is healthy.\\
\quad\textbf{Rank (G) 2}:  a salad is made up of these ingredients. every ingredient in a salad is healthy.\\
\quad\textbf{Rank 3}:  a salad is made up of these ingredients. every ingredient in a salad is unhealthy.\\
\quad\textbf{Rank 4}:  a salad is made up of these unhealthy ingredients. every ingredient in a salad is unhealthy.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_198}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  composition\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  The salad is healthy.\\
\textbf{Gold Premises}:  Every ingredient in a salad is healthy. A salad is made up of these ingredients.\\
\textbf{Rank}:  4\\
\quad\textbf{Rank 1}:  every ingredient in a salad is healthy. the salad contains at least one type of fruit.\\
\quad\textbf{Rank 2}:  a salad can be served as an appetizer or a main course. every ingredient in a salad is healthy.\\
\quad\textbf{Rank 3}:  a salad contains at least 3 different colors. every ingredient in a salad is healthy.\\
\quad\textbf{Rank (G) 4}:  every ingredient in a salad is healthy. a salad is made up of these ingredients.\\
\quad\textbf{Rank 5}:  the salad contains at least one type of fruit. every ingredient in a salad is organic.\\
\quad\textbf{Rank 6}:  a salad can be served as an appetizer or a main course. every ingredient in a salad is organic.\\
\quad\textbf{Rank 7}:  a salad is made up of these ingredients. every ingredient in a salad is organic.\\
\quad\textbf{Rank 8}:  a salad contains at least 3 different colors. every ingredient in a salad is organic.\\
\quad\textbf{Rank 9}:  every ingredient in a salad is grown outdoors. the salad contains at least one type of fruit.\\
\quad\textbf{Rank 10}:  every ingredient in a salad is available at the grocery store. the salad contains at least one type of fruit.\\
\quad\textbf{Rank 11}:  every ingredient in a salad is grown outdoors. a salad can be served as an appetizer or a main course.\\
\quad\textbf{Rank 12}:  every ingredient in a salad is available at the grocery store. a salad can be served as an appetizer or a main course.\\
\quad\textbf{Rank 13}:  every ingredient in a salad is grown outdoors. a salad contains at least 3 different colors.\\
\quad\textbf{Rank 14}:  every ingredient in a salad is grown outdoors. a salad is made up of these ingredients.\\
\quad\textbf{Rank 15}:  every ingredient in a salad is available at the grocery store. a salad is made up of these ingredients.\\
\quad\textbf{Rank 16}:  a salad contains at least 3 different colors. every ingredient in a salad is available at the grocery store.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_199}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  composition\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  The salad is healthy.\\
\textbf{Gold Premises}:  Every ingredient in a salad is healthy. A salad is made up of these ingredients.\\
\textbf{Rank}:  3\\
\quad\textbf{Rank 1}:  some ingredients in a salad are healthy. a salad is made up of only these healthy ingredients.\\
\quad\textbf{Rank 2}:  a salad is made up of only these healthy ingredients. every ingredient in a salad is healthy.\\
\quad\textbf{Rank (G) 3}:  a salad is made up of these ingredients. every ingredient in a salad is healthy.\\
\quad\textbf{Rank 4}:  a salad is made up of these ingredients. some ingredients in a salad are healthy.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_200}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  composition\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  The salad is healthy.\\
\textbf{Gold Premises}:  Every ingredient in a salad is healthy. A salad is made up of these ingredients.\\
\textbf{Rank}:  2\\
\quad\textbf{Rank 1}:  a salad is not made up of these healthy ingredients. every ingredient in a salad is healthy.\\
\quad\textbf{Rank (G) 2}:  a salad is made up of these ingredients. every ingredient in a salad is healthy.\\
\quad\textbf{Rank 3}:  not every ingredient in a salad is healthy. a salad is made up of these ingredients.\\
\quad\textbf{Rank 4}:  not every ingredient in a salad is healthy. a salad is not made up of these healthy ingredients.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_201}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  divisions\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  The individual players are skilled at playing offense and defense.\\
\textbf{Gold Premises}:  The football team is skilled at playing offense and defense. The individual players are part of the football team.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the individual players are part of the football team. the football team is skilled at playing offense and defense.\\
\quad\textbf{Rank 2}:  each player has never played football before. the football team is skilled at playing offense and defense.\\
\quad\textbf{Rank 3}:  the football team has never won a game before. the individual players are part of the football team.\\
\quad\textbf{Rank 4}:  the football team has never won a game before. each player has never played football before.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_238}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  divisions\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  The individual players are skilled at playing offense and defense.\\
\textbf{Gold Premises}:  The football team is skilled at playing offense and defense. The individual players are part of the football team.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the football team is skilled at playing offense and defense. the individual players are part of the football team.\\
\quad\textbf{Rank 2}:  the football team is skilled at playing offense and defense. each player has a favorite video game.\\
\quad\textbf{Rank 3}:  each player has a favorite food. the football team is skilled at playing offense and defense.\\
\quad\textbf{Rank 4}:  the football team is skilled at playing offense and defense. each player has a favorite type of sandwich.\\
\quad\textbf{Rank 5}:  the individual players are part of the football team. the football team practices on a grass field.\\
\quad\textbf{Rank 6}:  the football team practices at the local high school. the individual players are part of the football team.\\
\quad\textbf{Rank 7}:  the football team practices on a grass field. each player has a favorite video game.\\
\quad\textbf{Rank 8}:  the football team practices at the local high school. each player has a favorite video game.\\
\quad\textbf{Rank 9}:  each player has a favorite food. the football team practices on a grass field.\\
\quad\textbf{Rank 10}:  the football team practices at the local high school. each player has a favorite food.\\
\quad\textbf{Rank 11}:  each player has a favorite type of sandwich. the football team practices on a grass field.\\
\quad\textbf{Rank 12}:  the individual players are part of the football team. the football team has a team mascot.\\
\quad\textbf{Rank 13}:  the football team practices at the local high school. each player has a favorite type of sandwich.\\
\quad\textbf{Rank 14}:  each player has a favorite video game. the football team has a team mascot.\\
\quad\textbf{Rank 15}:  each player has a favorite food. the football team has a team mascot.\\
\quad\textbf{Rank 16}:  each player has a favorite type of sandwich. the football team has a team mascot.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_239}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  divisions\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  The individual players are skilled at playing offense and defense.\\
\textbf{Gold Premises}:  The football team is skilled at playing offense and defense. The individual players are part of the football team.\\
\textbf{Rank}:  2\\
\quad\textbf{Rank 1}:  all football teams are skilled at playing offense and defense. the individual players are part of the football team.\\
\quad\textbf{Rank (G) 2}:  the football team is skilled at playing offense and defense. the individual players are part of the football team.\\
\quad\textbf{Rank 3}:  the football team is skilled at playing offense and defense. some players are not part of the football team.\\
\quad\textbf{Rank 4}:  all football teams are skilled at playing offense and defense. some players are not part of the football team.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_240}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  divisions\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  The individual players are skilled at playing offense and defense.\\
\textbf{Gold Premises}:  The football team is skilled at playing offense and defense. The individual players are part of the football team.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the individual players are part of the football team. the football team is skilled at playing offense and defense.\\
\quad\textbf{Rank 2}:  each player is not part of the football team. the football team is skilled at playing offense and defense.\\
\quad\textbf{Rank 3}:  the individual players are part of the football team. the football team is not skilled at playing offense and defense.\\
\quad\textbf{Rank 4}:  the football team is not skilled at playing offense and defense. each player is not part of the football team.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_241}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  modus ponens\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  The temperature is warm.\\
\textbf{Gold Premises}:  If it's sunny, the temperature is warm. It's sunny.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  it's sunny. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 2}:  all players are part of the football team. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 3}:  it's sunny. all football teams are skilled at playing offense and defense.\\
\quad\textbf{Rank 4}:  all football teams are skilled at playing offense and defense. all players are part of the football team.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_278}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  modus ponens\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  The temperature is warm.\\
\textbf{Gold Premises}:  If it's sunny, the temperature is warm. It's sunny.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  it's sunny. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 2}:  each player has a favorite color. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 3}:  each player has a favorite type of car. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 4}:  each player has a favorite type of candy bar. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 5}:  it's sunny. the football team has a popular pre-game ritual.\\
\quad\textbf{Rank 6}:  the football team has a new coach this season. it's sunny.\\
\quad\textbf{Rank 7}:  the football team has a cheerleading squad. it's sunny.\\
\quad\textbf{Rank 8}:  the football team has a new coach this season. each player has a favorite color.\\
\quad\textbf{Rank 9}:  the football team has a new coach this season. each player has a favorite type of car.\\
\quad\textbf{Rank 10}:  each player has a favorite color. the football team has a popular pre-game ritual.\\
\quad\textbf{Rank 11}:  each player has a favorite color. the football team has a cheerleading squad.\\
\quad\textbf{Rank 12}:  each player has a favorite type of car. the football team has a popular pre-game ritual.\\
\quad\textbf{Rank 13}:  the football team has a new coach this season. each player has a favorite type of candy bar.\\
\quad\textbf{Rank 14}:  each player has a favorite type of car. the football team has a cheerleading squad.\\
\quad\textbf{Rank 15}:  the football team has a popular pre-game ritual. each player has a favorite type of candy bar.\\
\quad\textbf{Rank 16}:  the football team has a cheerleading squad. each player has a favorite type of candy bar.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_279}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  modus ponens\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  The temperature is warm.\\
\textbf{Gold Premises}:  If it's sunny, the temperature is warm. It's sunny.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  it's sunny. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 2}:  no player is part of the football team. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 3}:  some football teams are skilled at playing offense and defense. it's sunny.\\
\quad\textbf{Rank 4}:  some football teams are skilled at playing offense and defense. no player is part of the football team.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_280}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  modus ponens\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  The temperature is warm.\\
\textbf{Gold Premises}:  If it's sunny, the temperature is warm. It's sunny.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  it's sunny. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 2}:  a player is not part of the football team. if it's sunny, the temperature is warm.\\
\quad\textbf{Rank 3}:  not all football teams are skilled at playing offense and defense. it's sunny.\\
\quad\textbf{Rank 4}:  not all football teams are skilled at playing offense and defense. a player is not part of the football team.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_281}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  modus tollens\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  John is not at work.\\
\textbf{Gold Premises}:  If John is at work, he is not at home. John is at home.\\
\textbf{Rank}:  2\\
\quad\textbf{Rank 1}:  john is not at home. if john is at work, he is not at home.\\
\quad\textbf{Rank (G) 2}:  john is at home. if john is at work, he is not at home.\\
\quad\textbf{Rank 3}:  john is not at home. all those who work are at the office.\\
\quad\textbf{Rank 4}:  john is at home. all those who work are at the office.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_318}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  modus tollens\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  John is not at work.\\
\textbf{Gold Premises}:  If John is at work, he is not at home. John is at home.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  john is at home. if john is at work, he is not at home.\\
\quad\textbf{Rank 2}:  john wears glasses. if john is at work, he is not at home.\\
\quad\textbf{Rank 3}:  if john is at work, he is not at home. john has a cat named whiskers.\\
\quad\textbf{Rank 4}:  it is monday today. if john is at work, he is not at home.\\
\quad\textbf{Rank 5}:  john is at home. john is wearing a blue shirt.\\
\quad\textbf{Rank 6}:  john is at home. john ate a sandwich for lunch.\\
\quad\textbf{Rank 7}:  john drives a blue car. john is at home.\\
\quad\textbf{Rank 8}:  john has a cat named whiskers. john is wearing a blue shirt.\\
\quad\textbf{Rank 9}:  john wears glasses. john is wearing a blue shirt.\\
\quad\textbf{Rank 10}:  john wears glasses. john ate a sandwich for lunch.\\
\quad\textbf{Rank 11}:  it is monday today. john is wearing a blue shirt.\\
\quad\textbf{Rank 12}:  john ate a sandwich for lunch. john has a cat named whiskers.\\
\quad\textbf{Rank 13}:  john wears glasses. john drives a blue car.\\
\quad\textbf{Rank 14}:  john drives a blue car. john has a cat named whiskers.\\
\quad\textbf{Rank 15}:  it is monday today. john ate a sandwich for lunch.\\
\quad\textbf{Rank 16}:  it is monday today. john drives a blue car.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_319}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  modus tollens\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  John is not at work.\\
\textbf{Gold Premises}:  If John is at work, he is not at home. John is at home.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  if john is at work, he is not at home. john is at home.\\
\quad\textbf{Rank 2}:  if john is at work, he is not at home. some people at home are not on vacation.\\
\quad\textbf{Rank 3}:  john is at home. all who work are at the office.\\
\quad\textbf{Rank 4}:  some people at home are not on vacation. all who work are at the office.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_320}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  modus tollens\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  It is not a mammal.\\
\textbf{Gold Premises}:  If it is a mammal, it has fur. The animal has no fur.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  if it is a mammal, it has fur. the animal has no fur.\\
\quad\textbf{Rank 2}:  not all mammals have fur. the animal has no fur.\\
\quad\textbf{Rank 3}:  not all mammals have fur. the animal has fur.\\
\quad\textbf{Rank 4}:  if it is a mammal, it has fur. the animal has fur.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_324}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  definition\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  Basil is a plant used for flavoring, medicine, or fragrance.\\
\textbf{Gold Premises}:  An herb is a plant used for flavoring, medicine, or fragrance. Basil is an herb.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  basil is an herb. an herb is a plant used for flavoring, medicine, or fragrance.\\
\quad\textbf{Rank 2}:  basil is a type of insect. an herb is a plant used for flavoring, medicine, or fragrance.\\
\quad\textbf{Rank 3}:  a herb is a type of animal. basil is an herb.\\
\quad\textbf{Rank 4}:  a herb is a type of animal. basil is a type of insect.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_357}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  definition\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  Basil is a plant used for flavoring, medicine, or fragrance.\\
\textbf{Gold Premises}:  An herb is a plant used for flavoring, medicine, or fragrance. Basil is an herb.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  an herb is a plant used for flavoring, medicine, or fragrance. basil is an herb.\\
\quad\textbf{Rank 2}:  an herb is a plant used for flavoring, medicine, or fragrance. basil is native to tropical regions.\\
\quad\textbf{Rank 3}:  basil is an herb. basil is used in many cuisines around the world.\\
\quad\textbf{Rank 4}:  basil is used in many cuisines around the world. herbs have been used for medicinal purposes since ancient times.\\
\quad\textbf{Rank 5}:  basil is an herb. the scientific name for basil is ocimum basilicum.\\
\quad\textbf{Rank 6}:  basil is used in many cuisines around the world. herbs are often used to treat minor ailments.\\
\quad\textbf{Rank 7}:  basil is used in many cuisines around the world. basil is native to tropical regions.\\
\quad\textbf{Rank 8}:  basil is an herb. herbs are commonly used in italian cuisine.\\
\quad\textbf{Rank 9}:  herbs are commonly used in italian cuisine. basil is native to tropical regions.\\
\quad\textbf{Rank 10}:  basil is native to tropical regions. the scientific name for basil is ocimum basilicum.\\
\quad\textbf{Rank 11}:  an herb is a plant used for flavoring, medicine, or fragrance. herbs have been used for medicinal purposes since ancient times.\\
\quad\textbf{Rank 12}:  an herb is a plant used for flavoring, medicine, or fragrance. herbs are often used to treat minor ailments.\\
\quad\textbf{Rank 13}:  herbs have been used for medicinal purposes since ancient times. the scientific name for basil is ocimum basilicum.\\
\quad\textbf{Rank 14}:  herbs are often used to treat minor ailments. the scientific name for basil is ocimum basilicum.\\
\quad\textbf{Rank 15}:  herbs are commonly used in italian cuisine. herbs have been used for medicinal purposes since ancient times.\\
\quad\textbf{Rank 16}:  herbs are commonly used in italian cuisine. herbs are often used to treat minor ailments.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_358}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  definition\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  Basil is a plant used for flavoring, medicine, or fragrance.\\
\textbf{Gold Premises}:  An herb is a plant used for flavoring, medicine, or fragrance. Basil is an herb.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  basil is an herb. an herb is a plant used for flavoring, medicine, or fragrance.\\
\quad\textbf{Rank 2}:  all plants used for flavoring, medicine, or fragrance are herbs. basil is an herb.\\
\quad\textbf{Rank 3}:  some basil is not an herb. an herb is a plant used for flavoring, medicine, or fragrance.\\
\quad\textbf{Rank 4}:  some basil is not an herb. all plants used for flavoring, medicine, or fragrance are herbs.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_359}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  definition\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  Basil is a plant used for flavoring, medicine, or fragrance.\\
\textbf{Gold Premises}:  An herb is a plant used for flavoring, medicine, or fragrance. Basil is an herb.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  basil is an herb. an herb is a plant used for flavoring, medicine, or fragrance.\\
\quad\textbf{Rank 2}:  basil is not a herb. an herb is a plant used for flavoring, medicine, or fragrance.\\
\quad\textbf{Rank 3}:  not all plants used for flavoring, medicine, or fragrance are herbs. basil is an herb.\\
\quad\textbf{Rank 4}:  basil is not a herb. not all plants used for flavoring, medicine, or fragrance are herbs.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_360}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  temporal reasoning\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  I should leave at 7\\
\textbf{Gold Premises}:  The party starts at 8 PM. It takes 30 minutes to get there.\\
\textbf{Rank}:  3\\
\quad\textbf{Rank 1}:  it takes 30 minutes to get there. the party starts at 7 pm.\\
\quad\textbf{Rank 2}:  it takes 15 minutes to get there. the party starts at 7 pm.\\
\quad\textbf{Rank (G) 3}:  it takes 30 minutes to get there. the party starts at 8 pm.\\
\quad\textbf{Rank 4}:  it takes 15 minutes to get there. the party starts at 8 pm.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_397}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  temporal reasoning\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  I should leave at 7\\
\textbf{Gold Premises}:  The party starts at 8 PM. It takes 30 minutes to get there.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the party starts at 8 pm. it takes 30 minutes to get there.\\
\quad\textbf{Rank 2}:  it takes 30 minutes to get there. the party is a costume party.\\
\quad\textbf{Rank 3}:  it takes 30 minutes to get there. the party has a live band.\\
\quad\textbf{Rank 4}:  the party starts at 8 pm. the host is left-handed.\\
\quad\textbf{Rank 5}:  the party starts at 8 pm. the host is a teacher.\\
\quad\textbf{Rank 6}:  it takes 30 minutes to get there. the party has a pool.\\
\quad\textbf{Rank 7}:  the party starts at 8 pm. the host is allergic to peanuts.\\
\quad\textbf{Rank 8}:  the host is left-handed. the party is a costume party.\\
\quad\textbf{Rank 9}:  the host is a teacher. the party is a costume party.\\
\quad\textbf{Rank 10}:  the party has a live band. the host is left-handed.\\
\quad\textbf{Rank 11}:  the party has a live band. the host is a teacher.\\
\quad\textbf{Rank 12}:  the host is left-handed. the party has a pool.\\
\quad\textbf{Rank 13}:  the host is allergic to peanuts. the party is a costume party.\\
\quad\textbf{Rank 14}:  the host is a teacher. the party has a pool.\\
\quad\textbf{Rank 15}:  the host is allergic to peanuts. the party has a live band.\\
\quad\textbf{Rank 16}:  the host is allergic to peanuts. the party has a pool.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_398}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  temporal reasoning\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  I should leave at 7\\
\textbf{Gold Premises}:  The party starts at 8 PM. It takes 30 minutes to get there.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  it takes 30 minutes to get there. the party starts at 8 pm.\\
\quad\textbf{Rank 2}:  it takes 30 minutes to get there. all parties start at 8 pm.\\
\quad\textbf{Rank 3}:  some trips take 30 minutes to get there. the party starts at 8 pm.\\
\quad\textbf{Rank 4}:  some trips take 30 minutes to get there. all parties start at 8 pm.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_399}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  temporal reasoning\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  I should leave at 7\\
\textbf{Gold Premises}:  The party starts at 8 PM. It takes 30 minutes to get there.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  it takes 30 minutes to get there. the party starts at 8 pm.\\
\quad\textbf{Rank 2}:  the party does not start at 8 pm. it takes 30 minutes to get there.\\
\quad\textbf{Rank 3}:  it does not take 30 minutes to get there. the party starts at 8 pm.\\
\quad\textbf{Rank 4}:  it does not take 30 minutes to get there. the party does not start at 8 pm.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_400}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  propositional logic\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  The streets are wet.\\
\textbf{Gold Premises}:  It is raining outside. If it is raining, then the streets are wet.\\
\textbf{Rank}:  2\\
\quad\textbf{Rank 1}:  it is raining outside. if it is snowing, then the streets are wet.\\
\quad\textbf{Rank (G) 2}:  if it is raining, then the streets are wet. it is raining outside.\\
\quad\textbf{Rank 3}:  if it is raining, then the streets are wet. it is snowing outside.\\
\quad\textbf{Rank 4}:  if it is snowing, then the streets are wet. it is snowing outside.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_437}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  propositional logic\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  The streets are wet.\\
\textbf{Gold Premises}:  It is raining outside. If it is raining, then the streets are wet.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  if it is raining, then the streets are wet. it is raining outside.\\
\quad\textbf{Rank 2}:  if it is raining, then the streets are wet. there is a car parked outside.\\
\quad\textbf{Rank 3}:  if it is raining, then the streets are wet. my car needs new brakes.\\
\quad\textbf{Rank 4}:  if it is raining, then the streets are wet. my neighbor has a dog.\\
\quad\textbf{Rank 5}:  i like to wear rain boots on cloudy days. it is raining outside.\\
\quad\textbf{Rank 6}:  it is raining outside. i like to drink coffee when it rains.\\
\quad\textbf{Rank 7}:  there is a car parked outside. i like to wear rain boots on cloudy days.\\
\quad\textbf{Rank 8}:  there is a car parked outside. i like to drink coffee when it rains.\\
\quad\textbf{Rank 9}:  i like to wear a hat when it's cold. it is raining outside.\\
\quad\textbf{Rank 10}:  my car needs new brakes. i like to drink coffee when it rains.\\
\quad\textbf{Rank 11}:  i like to wear rain boots on cloudy days. my car needs new brakes.\\
\quad\textbf{Rank 12}:  i like to drink coffee when it rains. my neighbor has a dog.\\
\quad\textbf{Rank 13}:  there is a car parked outside. i like to wear a hat when it's cold.\\
\quad\textbf{Rank 14}:  i like to wear rain boots on cloudy days. my neighbor has a dog.\\
\quad\textbf{Rank 15}:  i like to wear a hat when it's cold. my car needs new brakes.\\
\quad\textbf{Rank 16}:  i like to wear a hat when it's cold. my neighbor has a dog.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_438}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  propositional logic\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  The streets are wet.\\
\textbf{Gold Premises}:  It is raining outside. If it is raining, then the streets are wet.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  if it is raining, then the streets are wet. it is raining outside.\\
\quad\textbf{Rank 2}:  if it is raining, then the streets are wet. all precipitation is rain.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_439}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  propositional logic\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  The streets are wet.\\
\textbf{Gold Premises}:  It is raining outside. If it is raining, then the streets are wet.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  it is raining outside. if it is raining, then the streets are wet.\\
\quad\textbf{Rank 2}:  if it is raining, then the streets are wet. it is not raining outside.\\
\quad\textbf{Rank 3}:  if it is not raining, then the streets are not wet. it is raining outside.\\
\quad\textbf{Rank 4}:  if it is not raining, then the streets are not wet. it is not raining outside.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_440}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  quantification logic\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  Some friendly dogs are black.\\
\textbf{Gold Premises}:  Some dogs are black. All black dogs are friendly.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  some dogs are black. all black dogs are friendly.\\
\quad\textbf{Rank 2}:  no dogs are black. all black dogs are friendly.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_476}
\end{mdframed}
\end{figure*}

\clearpage
\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  quantification logic\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  Some friendly dogs are black.\\
\textbf{Gold Premises}:  Some dogs are black. All black dogs are friendly.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  some dogs are black. all black dogs are friendly.\\
\quad\textbf{Rank 2}:  some dogs are black. the friendly black dogs weigh more than the unfriendly ones.\\
\quad\textbf{Rank 3}:  all black dogs are friendly. some dogs have brown eyes.\\
\quad\textbf{Rank 4}:  some dogs have brown eyes. the friendly black dogs weigh more than the unfriendly ones.\\
\quad\textbf{Rank 5}:  all black dogs are friendly. the basket is made of wicker.\\
\quad\textbf{Rank 6}:  some dogs are black. some of the apples in the basket were grown organically.\\
\quad\textbf{Rank 7}:  all black dogs are friendly. the apples were picked in the morning.\\
\quad\textbf{Rank 8}:  the basket is made of recycled materials. some dogs are black.\\
\quad\textbf{Rank 9}:  the basket is made of wicker. the friendly black dogs weigh more than the unfriendly ones.\\
\quad\textbf{Rank 10}:  the friendly black dogs weigh more than the unfriendly ones. the apples were picked in the morning.\\
\quad\textbf{Rank 11}:  some of the apples in the basket were grown organically. some dogs have brown eyes.\\
\quad\textbf{Rank 12}:  the basket is made of recycled materials. some dogs have brown eyes.\\
\quad\textbf{Rank 13}:  the basket is made of recycled materials. the apples were picked in the morning.\\
\quad\textbf{Rank 14}:  some of the apples in the basket were grown organically. the basket is made of wicker.\\
\quad\textbf{Rank 15}:  some of the apples in the basket were grown organically. the apples were picked in the morning.\\
\quad\textbf{Rank 16}:  the basket is made of recycled materials. the basket is made of wicker.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_477}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  quantification logic\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  Some friendly dogs are black.\\
\textbf{Gold Premises}:  Some dogs are black. All black dogs are friendly.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  all black dogs are friendly. some dogs are black.\\
\quad\textbf{Rank 2}:  all black dogs are friendly. some dogs are not black.\\
\quad\textbf{Rank 3}:  not all black dogs are friendly. some dogs are not black.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_478}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  quantification logic\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  Some friendly dogs are black.\\
\textbf{Gold Premises}:  Some dogs are black. All black dogs are friendly.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  all black dogs are friendly. some dogs are black.\\
\quad\textbf{Rank 2}:  not all black dogs are friendly. some dogs are black.\\
\quad\textbf{Rank 3}:  not all dogs are black. all black dogs are friendly.\\
\quad\textbf{Rank 4}:  not all dogs are black. not all black dogs are friendly.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_479}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  spatial reasoning\\
\textbf{Perturbation Type}:  FALSE PREMISE\\
\textbf{Target}:  The museum is northeast of the library.\\
\textbf{Gold Premises}:  The library is north of the park. The museum is east of the park.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the museum is east of the park. the library is north of the park.\\
\quad\textbf{Rank 2}:  the museum is west of the park. the library is north of the park.\\
\quad\textbf{Rank 3}:  the library is south of the park. the museum is east of the park.\\
\quad\textbf{Rank 4}:  the library is south of the park. the museum is west of the park.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_512}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  spatial reasoning\\
\textbf{Perturbation Type}:  IRRELEVANT FACT\\
\textbf{Target}:  The museum is northeast of the library.\\
\textbf{Gold Premises}:  The library is north of the park. The museum is east of the park.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the library is north of the park. the museum is east of the park.\\
\quad\textbf{Rank 2}:  the library has a red brick exterior. the museum is east of the park.\\
\quad\textbf{Rank 3}:  the library has a book drop on the side of the building. the museum is east of the park.\\
\quad\textbf{Rank 4}:  the library has a statue of a famous author in front of it. the museum is east of the park.\\
\quad\textbf{Rank 5}:  the library is north of the park. the museum has a café on the first floor.\\
\quad\textbf{Rank 6}:  the library is north of the park. the museum has a gift shop that sells postcards and souvenirs.\\
\quad\textbf{Rank 7}:  the library is north of the park. the museum has a volunteer program for high school students.\\
\quad\textbf{Rank 8}:  the library has a red brick exterior. the museum has a gift shop that sells postcards and souvenirs.\\
\quad\textbf{Rank 9}:  the museum has a café on the first floor. the library has a red brick exterior.\\
\quad\textbf{Rank 10}:  the library has a book drop on the side of the building. the museum has a café on the first floor.\\
\quad\textbf{Rank 11}:  the library has a book drop on the side of the building. the museum has a gift shop that sells postcards and souvenirs.\\
\quad\textbf{Rank 12}:  the library has a statue of a famous author in front of it. the museum has a café on the first floor.\\
\quad\textbf{Rank 13}:  the museum has a volunteer program for high school students. the library has a red brick exterior.\\
\quad\textbf{Rank 14}:  the library has a statue of a famous author in front of it. the museum has a gift shop that sells postcards and souvenirs.\\
\quad\textbf{Rank 15}:  the library has a book drop on the side of the building. the museum has a volunteer program for high school students.\\
\quad\textbf{Rank 16}:  the library has a statue of a famous author in front of it. the museum has a volunteer program for high school students.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_513}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  spatial reasoning\\
\textbf{Perturbation Type}:  Incorrect Quantifier\\
\textbf{Target}:  The museum is northeast of the library.\\
\textbf{Gold Premises}:  The library is north of the park. The museum is east of the park.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the museum is east of the park. the library is north of the park.\\
\quad\textbf{Rank 2}:  some museums are east of the park. the library is north of the park.\\
\quad\textbf{Rank 3}:  the museum is east of the park. all books in the library are north of the park.\\
\quad\textbf{Rank 4}:  all books in the library are north of the park. some museums are east of the park.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_514}
\end{mdframed}
\end{figure*}

\begin{figure*}
    \begin{mdframed}[backgroundcolor=gray!20, hidealllines=true]
    \centering
    \begin{tabular}{p{\linewidth-0.5cm}}



\textbf{Category}:  spatial reasoning\\
\textbf{Perturbation Type}:  NEGATED\\
\textbf{Target}:  The museum is northeast of the library.\\
\textbf{Gold Premises}:  The library is north of the park. The museum is east of the park.\\
\textbf{Rank}:  1\\
\quad\textbf{Rank (G) 1}:  the library is north of the park. the museum is east of the park.\\
\quad\textbf{Rank 2}:  the museum is east of the park. the library is not north of the park.\\
\quad\textbf{Rank 3}:  the library is north of the park. the museum is not east of the park.\\
\quad\textbf{Rank 4}:  the museum is not east of the park. the library is not north of the park.\\
\end{tabular}
\label{fig:ssrc_ranking_examples_515}
\end{mdframed}
\end{figure*}
